The Unreasonable Effectiveness of the Final Batch Normalization Layer

Early-stage disease indications are rarely recorded in real-world domains, such as Agriculture and Healthcare, and yet, their accurate identification is critical in that point of time. In this type of highly imbalanced classification problems, which encompass complex features, deep learning (DL) is much needed because of its strong detection capabilities. At the same time, DL is observed in practice to favor majority over minority classes and consequently suffer from inaccurate detection of the targeted early-stage indications. In this work, we extend the study done by Kocaman et al., 2020, showing that the final BN layer, when placed before the softmax output layer, has a considerable impact in highly imbalanced image classification problems as well as undermines the role of the softmax outputs as an uncertainty measure. This current study addresses additional hypotheses and reports on the following findings: (i) the performance gain after adding the final BN layer in highly imbalanced settings could still be achieved after removing this additional BN layer in inference; (ii) there is a certain threshold for the imbalance ratio upon which the progress gained by the final BN layer reaches its peak; (iii) the batch size also plays a role and affects the outcome of the final BN application; (iv) the impact of the BN application is also reproducible on other datasets and when utilizing much simpler neural architectures; (v) the reported BN effect occurs only per a single majority class and multiple minority classes i.e., no improvements are evident when there are two majority classes; and finally, (vi) utilizing this BN layer with sigmoid activation has almost no impact when dealing with a strongly imbalanced image classification tasks.

==> RelatedWork.tex <==
\section{Related Work}
\label{sec:relatedWork}
Investigating the effect of learnable parameters of BN, scale ($\gamma$) and shift ($\beta$), on the training of various typical deep neural nets, Wang et al.~\citep{wang2018batch} suggest that there is no big difference in both training convergence and final test accuracy when removing the BN layer following the final convolutional layer from a convolutional neural network (CNN) for standard classification tasks. The authors claim that it is not necessary to adjust the learnable gain and bias along the training process and they show that the use of constant gain and bias is enough and these learneable parameters have little effect on the performance. They also observe that without adaptively updating learnable parameters for BN layers, it often requires less time for training of very deep neural nets such as ResNet-101. 

Frankle et al.~\citep{frankle2020training} also studied the effect of learnable BN parameters, showing that BN’s trainable parameters alone can account for much of a network’s accuracy. They found that,
when locking all other layers at their random initial weights and then training the network for fifty or so epochs, it will perform better than random. As it adjusts a network’s intermediate feature representations for a given mini batch, BN itself learns how to do so in a consistent way for all mini batches. The researchers probed the impact of this learning by training only the BN parameters, $\gamma$ and $\beta$, while setting all other parameters at random.   

Bjorck et al.~\citep{bjorck2018understanding} conducted another experiment, similar to our study. They trained a ResNet that uses one BN layer only at the very last convolutional layer of the network (removing all the other BN layers coming after each CNN layer), normalizing the output of the last residual block but without intermediate activation. This indicates that after initialization, the network tends to almost always predict the same (typically wrong) class, which is then corrected with a strong gradient update. In contrast, the network with BN does not exhibit the same behavior; rather, positive gradients are distributed throughout all classes. Their findings suggest that normalizing the final layer of a deep network may be one of the most important contributions of BN. 

Zhu et al.~\citep{zhu2020improving} adopted a similar idea of using the \textit{scalable version of a BN layer} to normalize the channel at the final output of the network, and improving the classification performance of softmax \textit{without adding learnable BN parameters}, but controlling the output distribution by another scaling parameter. However, their improvements on selected datasets were not significant (less then 0.3\%).

Yasuda et al.~\citep{yasuda2020consistent} worked on the combination of weighted loss function (WLF) and BN to improve learning in imbalanced-data environment, but their main goal was to resolve the size-inconsistency problem which arises in the combination of WLF and BN in a standard feed forward neural networks.

Apart from these studies, to the best of our knowledge, there is no prior work investigating the effect of BN utilization over imbalanced image classification tasks when set before the softmax output layer.
%\tb{Maybe, after the initial introduction of the abbreviation, just always write "BN"?}\tb {(vk) yes, I will do that all over the paper}

 

